Gluon correlation functions from lattice quantum chromodynamics

We study the gluon sector in pure Yang-Mills theories via the computation of two, three and four point Landau gauge gluon correlation functions via LQCD using the Wilson action for Monte-Carlo simulations. The first goal was to use lattice tensor representations for the propagator in four dimensions to understand/quantify deviations of the lattice propagator from its continuum form. We also identified classes of kinematic configurations where these deviations are minimal and the continuum description of lattice tensors is improved. These tensor structures also allow to verify that the continuum Slavnov-Taylor identity for the propagator is is fulfilled, with good accuracy, on the lattice. The computation of the three gluon vertex served to explore the so-called zero crossing, a property related to the ghost dominance at the infrared scales that restricts the behaviour of the three gluon vertex. We also explore the possible existence of a ghost mass preventing the IR divergence. Functional forms were used to model the lattice data and explore the two different possibilities for the IR behaviour. In the first case we estimate the mass scale associated with the crossing and search for a possible sign of the divergence. Secondly, we study the possibility of a sign change and a finite zero momentum value of the vertex. A last topic is the calculation of the four gluon vertex. A suitable choice of kinematics allows to eliminate the unwanted contributions from lower order functions while large statistical fluctuations hinder the precise computation of this object. Our investigation is a proof of concept, we show that the lattice computation of the four gluon correlation function is feasible with reasonable computational resources. An increase in statistics is necessary to provide a clearer signal on the complete correlation function and to compute the one particle irreducible function.

==> analysis_results/Propagator/plots/64_continuum_relations_diag.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,3374.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(467,562){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(467,829){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(467,1096){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,1363){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(467,1631){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(467,1898){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \put(467,2165){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(467,2432){\makebox(0,0)[r]{\strut{}$3.5$}}%
      \put(467,2699){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(599,342){\makebox(0,0){\strut{}$0$}}%
      \put(1001,342){\makebox(0,0){\strut{}$0.5$}}%
      \put(1404,342){\makebox(0,0){\strut{}$1$}}%
      \put(1806,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(2208,342){\makebox(0,0){\strut{}$2$}}%
      \put(2611,342){\makebox(0,0){\strut{}$2.5$}}%
      \put(3013,342){\makebox(0,0){\strut{}$3$}}%
      \put(3415,342){\makebox(0,0){\strut{}$3.5$}}%
      \put(3818,342){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(995,776){\makebox(0,0)[l]{\strut{}$\scriptscriptstyle (n,n,n,n)$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-149,1630){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle p^2\Gamma(p^2)$}}}%
      \put(2248,12){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \put(3373,2526){\makebox(0,0)[r]{\strut{}$\scriptstyle d(\hat p^2)$}}%
      \csname LTb\endcsname%%
      \put(3373,2306){\makebox(0,0)[r]{\strut{}$\scriptstyle (E(\hat p^2)+n^2F(\hat p^2) + n^4G(\hat p^2))\frac{4}{3}\hat p^2$}}%
      \csname LTb\endcsname%%
      \put(3373,2086){\makebox(0,0)[r]{\strut{}$\scriptstyle -p^2H(\hat p^2) - p^4I(\hat p^2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4048,342){\makebox(0,0){\strut{}$0$}}%
      \put(4723,342){\makebox(0,0){\strut{}$0.5$}}%
      \put(5398,342){\makebox(0,0){\strut{}$1$}}%
      \put(6072,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(6747,342){\makebox(0,0){\strut{}$2$}}%
      \put(7422,342){\makebox(0,0){\strut{}$2.5$}}%
      \csname LTb\endcsname%%
      \put(4453,776){\makebox(0,0)[l]{\strut{}$\scriptscriptstyle (n,0,0,0)$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5735,12){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \put(6897,2526){\makebox(0,0)[r]{\strut{}$\scriptstyle d(\hat p^2)$}}%
      \csname LTb\endcsname%%
      \put(6897,2306){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2D(\hat p^2)$}}%
      \csname LTb\endcsname%%
      \put(6897,2086){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2E(\hat p^2)$}}%
      \csname LTb\endcsname%%
      \put(6897,1866){\makebox(0,0)[r]{\strut{}$\scriptstyle -\hat p^4F(\hat p^2) -\hat p^4G(\hat p^2)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{64_continuum_relations_diag}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/GI_factors_nocorrection.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,3374.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(467,704){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(467,1317){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(467,1929){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(467,2542){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(467,3154){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(773,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(1120,484){\makebox(0,0){\strut{}$1.4$}}%
      \put(1467,484){\makebox(0,0){\strut{}$1.6$}}%
      \put(1814,484){\makebox(0,0){\strut{}$1.8$}}%
      \put(2162,484){\makebox(0,0){\strut{}$2$}}%
      \put(2509,484){\makebox(0,0){\strut{}$2.2$}}%
      \put(2856,484){\makebox(0,0){\strut{}$2.4$}}%
      \put(3203,484){\makebox(0,0){\strut{}$2.6$}}%
      \put(3551,484){\makebox(0,0){\strut{}$2.8$}}%
      \put(3898,484){\makebox(0,0){\strut{}$3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-281,1929){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle\Gamma(p^2)$}}}%
      \put(2248,154){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(2911,2981){\makebox(0,0)[r]{\strut{}$\hat p^4I(\hat p^2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4222,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(4569,484){\makebox(0,0){\strut{}$1.4$}}%
      \put(4916,484){\makebox(0,0){\strut{}$1.6$}}%
      \put(5263,484){\makebox(0,0){\strut{}$1.8$}}%
      \put(5611,484){\makebox(0,0){\strut{}$2$}}%
      \put(5958,484){\makebox(0,0){\strut{}$2.2$}}%
      \put(6305,484){\makebox(0,0){\strut{}$2.4$}}%
      \put(6652,484){\makebox(0,0){\strut{}$2.6$}}%
      \put(7000,484){\makebox(0,0){\strut{}$2.8$}}%
      \put(7347,484){\makebox(0,0){\strut{}$3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5697,154){\makebox(0,0){\strut{}$p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(6360,2981){\makebox(0,0)[r]{\strut{}$p^4I(p^2)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{GI_factors_nocorrection}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/form_factors_lattice_H4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,5624.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(392,3261){\makebox(0,0)[r]{\strut{}$-15$}}%
      \put(392,3617){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(392,3973){\makebox(0,0)[r]{\strut{}$-5$}}%
      \put(392,4330){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(392,4686){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(392,5042){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(392,5398){\makebox(0,0)[r]{\strut{}$15$}}%
      \put(611,3041){\makebox(0,0){\strut{}$1$}}%
      \put(1049,3041){\makebox(0,0){\strut{}$1.5$}}%
      \put(1486,3041){\makebox(0,0){\strut{}$2$}}%
      \put(1924,3041){\makebox(0,0){\strut{}$2.5$}}%
      \put(2361,3041){\makebox(0,0){\strut{}$3$}}%
      \put(2798,3041){\makebox(0,0){\strut{}$3.5$}}%
      \put(3236,3041){\makebox(0,0){\strut{}$4$}}%
      \put(3673,3041){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-224,4329){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle\Gamma(p^2)$}}}%
      \csname LTb\endcsname%%
      \put(2661,3899){\makebox(0,0)[r]{\strut{}$\scriptstyle E(p^2)$}}%
      \csname LTb\endcsname%%
      \put(2661,3679){\makebox(0,0)[r]{\strut{}$\scriptstyle p^2F(p^2)$}}%
      \csname LTb\endcsname%%
      \put(2661,3459){\makebox(0,0)[r]{\strut{}$\scriptstyle p^2H(p^2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4141,3261){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(4141,3528){\makebox(0,0)[r]{\strut{}$-1.5$}}%
      \put(4141,3795){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(4141,4062){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(4141,4330){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(4141,4597){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(4141,4864){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(4141,5131){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(4141,5398){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(4360,3041){\makebox(0,0){\strut{}$1$}}%
      \put(4798,3041){\makebox(0,0){\strut{}$1.5$}}%
      \put(5235,3041){\makebox(0,0){\strut{}$2$}}%
      \put(5673,3041){\makebox(0,0){\strut{}$2.5$}}%
      \put(6110,3041){\makebox(0,0){\strut{}$3$}}%
      \put(6547,3041){\makebox(0,0){\strut{}$3.5$}}%
      \put(6985,3041){\makebox(0,0){\strut{}$4$}}%
      \put(7422,3041){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(6410,3899){\makebox(0,0)[r]{\strut{}$\scriptstyle p^4G(p^2)$}}%
      \csname LTb\endcsname%%
      \put(6410,3679){\makebox(0,0)[r]{\strut{}$\scriptstyle p^4I(p^2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1967,562){\makebox(0,0)[r]{\strut{}$-15$}}%
      \put(1967,918){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(1967,1274){\makebox(0,0)[r]{\strut{}$-5$}}%
      \put(1967,1631){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1967,1987){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(1967,2343){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1967,2699){\makebox(0,0)[r]{\strut{}$15$}}%
      \put(2191,342){\makebox(0,0){\strut{}$1$}}%
      \put(2649,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(3107,342){\makebox(0,0){\strut{}$2$}}%
      \put(3565,342){\makebox(0,0){\strut{}$2.5$}}%
      \put(4023,342){\makebox(0,0){\strut{}$3$}}%
      \put(4481,342){\makebox(0,0){\strut{}$3.5$}}%
      \put(4939,342){\makebox(0,0){\strut{}$4$}}%
      \put(5397,342){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1351,1630){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle\Gamma(p^2)$}}}%
      \put(3748,12){\makebox(0,0){\strut{}$p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(4377,1200){\makebox(0,0)[r]{\strut{}$\scriptstyle J(p^2)$}}%
      \csname LTb\endcsname%%
      \put(4377,980){\makebox(0,0)[r]{\strut{}$\scriptstyle p^2K(p^2)$}}%
      \csname LTb\endcsname%%
      \put(4377,760){\makebox(0,0)[r]{\strut{}$\scriptstyle p^2L(p^2)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{form_factors_lattice_H4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/form_factors_lattice_IMP.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,5624.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(392,3261){\makebox(0,0)[r]{\strut{}$-15$}}%
      \put(392,3617){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(392,3973){\makebox(0,0)[r]{\strut{}$-5$}}%
      \put(392,4330){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(392,4686){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(392,5042){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(392,5398){\makebox(0,0)[r]{\strut{}$15$}}%
      \put(611,3041){\makebox(0,0){\strut{}$1$}}%
      \put(1049,3041){\makebox(0,0){\strut{}$1.5$}}%
      \put(1486,3041){\makebox(0,0){\strut{}$2$}}%
      \put(1924,3041){\makebox(0,0){\strut{}$2.5$}}%
      \put(2361,3041){\makebox(0,0){\strut{}$3$}}%
      \put(2798,3041){\makebox(0,0){\strut{}$3.5$}}%
      \put(3236,3041){\makebox(0,0){\strut{}$4$}}%
      \put(3673,3041){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-224,4329){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle\Gamma(p^2)$}}}%
      \csname LTb\endcsname%%
      \put(2661,3899){\makebox(0,0)[r]{\strut{}$\scriptstyle E(\hat p^2) $}}%
      \csname LTb\endcsname%%
      \put(2661,3679){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2 F(\hat p^2) $}}%
      \csname LTb\endcsname%%
      \put(2661,3459){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2 H(\hat p^2) $}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4141,3261){\makebox(0,0)[r]{\strut{}$-1.5$}}%
      \put(4141,3566){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(4141,3872){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(4141,4177){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(4141,4482){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(4141,4787){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(4141,5093){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(4141,5398){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(4360,3041){\makebox(0,0){\strut{}$1$}}%
      \put(4798,3041){\makebox(0,0){\strut{}$1.5$}}%
      \put(5235,3041){\makebox(0,0){\strut{}$2$}}%
      \put(5673,3041){\makebox(0,0){\strut{}$2.5$}}%
      \put(6110,3041){\makebox(0,0){\strut{}$3$}}%
      \put(6547,3041){\makebox(0,0){\strut{}$3.5$}}%
      \put(6985,3041){\makebox(0,0){\strut{}$4$}}%
      \put(7422,3041){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(6410,3899){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^4 G(\hat p^2) $}}%
      \csname LTb\endcsname%%
      \put(6410,3679){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^4 I(\hat p^2) $}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1967,562){\makebox(0,0)[r]{\strut{}$-15$}}%
      \put(1967,918){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(1967,1274){\makebox(0,0)[r]{\strut{}$-5$}}%
      \put(1967,1631){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1967,1987){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(1967,2343){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1967,2699){\makebox(0,0)[r]{\strut{}$15$}}%
      \put(2191,342){\makebox(0,0){\strut{}$1$}}%
      \put(2649,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(3107,342){\makebox(0,0){\strut{}$2$}}%
      \put(3565,342){\makebox(0,0){\strut{}$2.5$}}%
      \put(4023,342){\makebox(0,0){\strut{}$3$}}%
      \put(4481,342){\makebox(0,0){\strut{}$3.5$}}%
      \put(4939,342){\makebox(0,0){\strut{}$4$}}%
      \put(5397,342){\makebox(0,0){\strut{}$4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1351,1630){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle\Gamma(p^2)$}}}%
      \put(3748,12){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(4377,1200){\makebox(0,0)[r]{\strut{}$\scriptstyle J(\hat p^2) $}}%
      \csname LTb\endcsname%%
      \put(4377,980){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2 K(\hat p^2) $}}%
      \csname LTb\endcsname%%
      \put(4377,760){\makebox(0,0)[r]{\strut{}$\scriptstyle \hat p^2 L(\hat p^2) $}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{form_factors_lattice_IMP}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/orthogonality_general.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,3374.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(92,704){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(92,1317){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(92,1929){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(92,2542){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(92,3154){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(394,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(733,484){\makebox(0,0){\strut{}$1.4$}}%
      \put(1072,484){\makebox(0,0){\strut{}$1.6$}}%
      \put(1412,484){\makebox(0,0){\strut{}$1.8$}}%
      \put(1751,484){\makebox(0,0){\strut{}$2$}}%
      \put(2091,484){\makebox(0,0){\strut{}$2.2$}}%
      \put(2430,484){\makebox(0,0){\strut{}$2.4$}}%
      \put(2769,484){\makebox(0,0){\strut{}$2.6$}}%
      \put(3109,484){\makebox(0,0){\strut{}$2.8$}}%
      \put(3448,484){\makebox(0,0){\strut{}$3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1836,154){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(2923,2981){\makebox(0,0)[r]{\strut{}$\hat p^4I(\hat p^2)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3841,704){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(3841,1317){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(3841,1929){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(3841,2542){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(3841,3154){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(4135,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(4458,484){\makebox(0,0){\strut{}$1.4$}}%
      \put(4782,484){\makebox(0,0){\strut{}$1.6$}}%
      \put(5106,484){\makebox(0,0){\strut{}$1.8$}}%
      \put(5429,484){\makebox(0,0){\strut{}$2$}}%
      \put(5753,484){\makebox(0,0){\strut{}$2.2$}}%
      \put(6076,484){\makebox(0,0){\strut{}$2.4$}}%
      \put(6400,484){\makebox(0,0){\strut{}$2.6$}}%
      \put(6723,484){\makebox(0,0){\strut{}$2.8$}}%
      \put(7047,484){\makebox(0,0){\strut{}$3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5510,154){\makebox(0,0){\strut{}$p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(6522,2981){\makebox(0,0)[r]{\strut{}$p^4I(p^2)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{orthogonality_general}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/ratio_volumes.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7498.00,3374.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(467,562){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,870){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,1177){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,1502){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,1810){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,2118){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(467,2425){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(599,342){\makebox(0,0){\strut{}$0$}}%
      \put(1011,342){\makebox(0,0){\strut{}$0.5$}}%
      \put(1424,342){\makebox(0,0){\strut{}$1$}}%
      \put(1836,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(2249,342){\makebox(0,0){\strut{}$2$}}%
      \put(2661,342){\makebox(0,0){\strut{}$2.5$}}%
      \put(3073,342){\makebox(0,0){\strut{}$3$}}%
      \put(3486,342){\makebox(0,0){\strut{}$3.5$}}%
      \put(3898,342){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(995,776){\makebox(0,0)[l]{\strut{}$\scriptscriptstyle (n,n,n,n)$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(115,1630){\rotatebox{-270}{\makebox(0,0){\strut{}$\scriptstyle p^2\Gamma(p^2)$}}}%
      \put(2248,12){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(3373,2526){\makebox(0,0)[r]{\strut{}$\scriptstyle 80^4 -- EFG/HI$}}%
      \csname LTb\endcsname%%
      \put(3373,2306){\makebox(0,0)[r]{\strut{}$\scriptstyle 64^4 -- EFG/HI$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4048,342){\makebox(0,0){\strut{}$0$}}%
      \put(4470,342){\makebox(0,0){\strut{}$0.5$}}%
      \put(4892,342){\makebox(0,0){\strut{}$1$}}%
      \put(5313,342){\makebox(0,0){\strut{}$1.5$}}%
      \put(5735,342){\makebox(0,0){\strut{}$2$}}%
      \put(6157,342){\makebox(0,0){\strut{}$2.5$}}%
      \put(6579,342){\makebox(0,0){\strut{}$3$}}%
      \put(7000,342){\makebox(0,0){\strut{}$3.5$}}%
      \put(7422,342){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(4453,776){\makebox(0,0)[l]{\strut{}$\scriptscriptstyle (n,0,0,0)$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5735,12){\makebox(0,0){\strut{}$\hat p~(\si{GeV})$}}%
      \csname LTb\endcsname%%
      \put(6897,2526){\makebox(0,0)[r]{\strut{}$\scriptstyle 80^4 -- EFG/HI$}}%
      \csname LTb\endcsname%%
      \put(6897,2306){\makebox(0,0)[r]{\strut{}$\scriptstyle 80^4 -- EFG/HI$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ratio_volumes}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> analysis_results/Propagator/plots/save <==
set size 1,1.2
set origin 0,0
set multiplot
set size 0.5,0.5
unset xlabel
#################################################################################################### (4m,m,m,0) - IMPROVED LATTICE BASIS
set origin 0,0.5
set lmargin at screen 0.04
set rmargin at screen 0.48
set label "$\\scriptscriptstyle a)$"  at graph 0.05, 0.1
set label "$\\scriptscriptstyle (4m,m,m,0)$"  at graph 0.12, 0.1
condition1 = '($1 == 4*$2 && $2 == $3 && $4 == 0)'
set yrange[0:3]
set autoscale
set xrange [1:4]
plot @D1_IMP, @E1_IMP, @p2F1_IMP, @p2H1_IMP
unset label
#################################################################################################### (4m,m,m,0) - NORMAL MOMENTUM LATTICE BASIS
set origin 0.5,0.5
unset ylabel
unset ytics
set lmargin at screen 0.5
set rmargin at screen 0.94
set label "$\\scriptscriptstyle b)$"  at graph 0.05, 0.1
set label "$\\scriptscriptstyle (4m,m,m,0)$"  at graph 0.12, 0.1
condition1 = '($1 == 4*$2 && $2 == $3 && $4 == 0)'
set yrange[0:3]
set autoscale
set xrange [1:4]
plot @D1, @E1, @p2F1, @p2H1
unset label
#################################################################################################### (m+1,m,m,m-1)
unset key
set origin 0,0
set ytics
set lmargin at screen 0.04
set rmargin at screen 0.48
#set bmargin at screen 0.1
set xlabel "$\\hat p~(\\si{GeV})$"
unset key
set label "$\\scriptscriptstyle c)$"  at graph 0.05, 0.1
set label "$\\scriptscriptstyle p=(m+6,m,m,m-6)$" at graph 0.12,0.1
condition1 = '($1 == $2+6 && $3 == $2 && $4 == $2-6)'
set autoscale
set yrange[0.4:1.9]
set xrange [2:3.5]
plot @D1_IMP, @E1_IMP, @p2F1_IMP, @p2H1_IMP
unset label
#################################################################################################### (m+6,m,m,m-6)
set origin 0.5,0
unset ylabel
unset ytics
set key
set lmargin at screen 0.5
set rmargin at screen 0.94
#set bmargin at screen 0.1
set xlabel "$p~(\\si{GeV})$"
unset key
set label "$\\scriptscriptstyle d)$"  at graph 0.05, 0.1
set label "$\\scriptscriptstyle p=(m+6,m,m,m-6)$" at graph 0.12,0.1
condition1 = '($1 == $2+6 && $3 == $2 && $4 == $2-6)'
set autoscale
set yrange[0.4:1.9]
set xrange [2:3.5]
plot @D1, @E1, @p2F1, @p2H1
unset label
####################################################################################################
unset multiplot
set output

==> intro_lqcd/intro_lqcd_1.tex <==
In this chapter the formulation of quantum chromodynamics on a finite discretized lattice will be presented. With the use of imaginary time formalism, this allows the use of numerical simulations to study the non-perturbative regime of QCD.
The lattice alto cuts of the high frequency modes thus regularizing the theory. This was first suggested by Wilson in 1974 \cite{Wilson1974}.


This chapter begins with the introduction of the lattice formalism, constructing all objects in the discretized framework. After this, attention will be given to some computational aspects which are necessary to compute lattice quantities. For a presentation on the subject we recommend \cite{Wilson1974,Rothe,Gattringer2010}.

\section{Euclidean formulation}\label{sec:euclidean formulation}

The Minkowski space-time is not convenient to perform the functional path integrals due to the oscillatory behaviour of the exponential in the action. We use the imaginary time thus becoming an Euclidean space. This is accomplished by a Wick rotation, where the time is rotated by $\pi/2$ into the complex plane, $\tau=it$ where $t$ is the real time.
The exponential becomes similar to the Boltzmann factor on the partition function of statistical mechanics,
\begin{equation*}
\int\mathcal{D}\phi e^{iS[\phi]} \rightarrow \int\mathcal{D}e^{-S_E[\phi]}.
\end{equation*}
The object $S_E$ is the Euclidean version of the action, obtained by performing the change of variables above.
It is this observation, establishing the connection with statistical mechanics that allows methods used in this subject to be applied on lattice field theories, notably Monte-Carlo methods to obtain correlation functions. %It can be now noticed that the analogy with statistical mechanics is more evident when using the path integral approach to quantization.
In the forthcoming analysis we consider the Euclidean formulation of QCD, the metric is thus equivalent to $\delta_{\mu\nu}$ and so we do not distinguish upper and lower indices.

For completeness, we refer that this analytic continuation to the Euclidean space-time is not always trivial and it is related to the Hamiltonian of the theory being a non-negative, self-adjoint operator acting on the Hilbert space which is necessary for a quantum theory. The conditions for the proper definition of the Euclidean theory and the analytic continuation back to Minkowski space to be possible are given by the \textit{Osterwalder-Schrader} axioms \cite{Osterwalder1973}, reviewed in \cite{montvay_1994}. The cases considered in this work satisfy these conditions and this technical detail will not be relevant.



\section{Discretization}


In the lattice formulation the continuous space-time is replaced by a 4-dimensional Euclidean lattice $\Lambda$ with spacing $a$ where each point is labelled by four integers, $n = (n_1,n_2,n_3,n_4)$. In this work the lattice is hypercubic each side having the same number of points, $n_i\in[-N/2+1,N/2]$. The lattice $\Lambda$ is defined by
\begin{equation}
	\Lambda = \{x_\mu = an_\mu | n_\mu\in\mathds{Z}, |n_\mu|< N/2, \mu = 1,2,3,4\}
\end{equation}
where $n_4$ corresponds to the imaginary time direction.

The objects appearing in the continuum theory must be rewritten on the lattice formulation. For a general quantum field theory with fields $\phi$, the degrees of freedom are the classical fields $\phi(an)$ in the discrete lattice sites. The action must be correctly built in the new formalism in order to preserve all possible key properties of the continuum theory. The discretization procedure is not unique and this can be easily seen by the structure of the discrete derivative, taking various possible forms,
\begin{align}
&\partial_\mu\phi(x) = \frac{1}{a}\left(\phi(x+\hat\mu a) - \phi(x)\right) + \order{a}\\
&\partial_\mu\phi(x) = \frac{1}{2a}\left(\phi(x+\hat\mu a) - \phi(x-\hat\mu a)\right) + \order{a^2}.
\end{align}
This freedom in obtaining the lattice form should be used to minimize the appearance of lattice artifacts, however certain properties are unavoidably lost. It also opens the possibility for \textit{improvement schemes} which modify the action in a way to reduce lattice artifacts \cite{HASENFRATZ199853} -- these are not considered in this work. %This is the case of Poincaré group symmetry, being replaced by a discrete group. In the Euclidean formulation the $O(4)$ group symmetry of space is replaced by the hypercubic group, $H(4)$. These matters will be properly considered in chapter \ref{chap:tensorbases}.

An important consequence of the discretization of space-time, related to the discrete group symmetry surviving discretization is the fact that translations have to be at least one lattice unit, which results in the discretization of the allowed momenta. To see this consider the usual continuum Fourier transform,
\begin{equation*}
\phi(x) = \int\frac{d^4p}{(2\pi)^4}\tilde\phi(p)e^{ipx}.
\end{equation*}
Since $x = an$ is an integer multiple of the spacing $a$
\begin{equation*}
e^{ip_\mu x_\mu} = e^{i(p_\mu x_\mu + 2\pi n_\mu)} = e^{i(p_\mu + 2\pi/a)x_\mu},
\end{equation*}
the momentum $p_\mu$ is equivalent to $p_\mu + 2\pi/a$, allowing us to restrict the integration to the Brillouin zone, $-\pi/a < p_\mu \leq \pi/a$. This results in the removal of high frequency modes making the theory regularized.

In the infinite volume we would write
\begin{equation*}
\phi(x) = \int_{-\pi/a}^{\pi/a}\frac{d^4p}{(2\pi)^4}\tilde\phi(p)e^{ipx}.
\end{equation*}
To perform numerical simulations the volume of the lattice is finite, where we impose some kind of boundary conditions, $\phi(x + \hat\mu N_\mu a) = e^{i\theta_\mu}\phi(x)$. As usual, the finite volume also imposes the discretization of momentum which can be extracted from the Fourier transform of this condition,
\begin{align*}
\int_{-\pi/a}^{\pi/a}\frac{d^4p}{(2\pi)^4}\tilde\phi(p)e^{ip_\mu(x_\mu + \hat\mu N_\mu a)} &= \int_{-\pi/a}^{\pi/a}\frac{d^4p}{(2\pi)^4}\tilde\phi(p)e^{ip_\mu x_\mu+i\theta_\mu} \\
\Leftrightarrow e^{ip_\mu N_\mu} &= e^{i\theta_\mu}~ (\text{no sum})
\end{align*}
where $\hat\mu$ is an unitary lattice vector in the direction $\mu$.
From this we have the possible discretized momentum in a lattice with undefined boundary conditions
\begin{equation*}
p_\mu = \frac{2\pi n_\mu}{aN_\mu}+\frac{\theta_\mu}{aN_\mu}.
\end{equation*}
In this work the fields satisfy periodic boundary conditions, thus $\theta_\mu = 0$ and we get the discrete momentum values,
\begin{equation}
p_\mu = \frac{2\pi n_\mu}{aN_\mu}, ~n_\mu\in\{-N_\mu/2+1, ..., N_\mu/2\}.
\label{eq:lattice_momenta}
\end{equation}
Notice how the use of a finite volume relates to the lowest momentum attainable for a given lattice and also to its resolution.
As usual, having a finite number of momenta available, the discrete Fourier transform becomes the sum,
\begin{equation*}
\phi(x) = \frac{1}{V}\sum_{n_\mu = -N/2+1}^{N/2}\tilde\phi(p_n)e^{ip_n\cdot x}
\end{equation*}
where $V = N^4$ is the volume of the space-time grid for the hypercubic lattice.

Other than the continuum discretized momentum \eqref{eq:lattice_momenta}, in this work we will also consider the lattice perturbation theory \cite{CAPITANI_perturb} improved momentum defined by
\begin{equation}
\hat p_\mu = 2\sin\left(\frac{ap_\mu}{2}\right) = 2\sin\left(\frac{\pi n_\mu}{N}\right).
\label{eq:improved_momenta}
\end{equation}
This form also appears in the computation of the tree-level propagator of a massless scalar field in the lattice. This replacement does not deliver significant changes for low momentum, but it should be manifest for higher momentum. In \cref{chap:tensorbases} we will see how this momentum arises when considering the most general form of a vector for the lattice symmetry and how it takes into account the lattice artifacts in the tensor description.

The general path integral quantization scheme is built analogously to the continuum formulation. The partition function is constructed 
\begin{equation}
\mathcal{Z} = \int \mathcal{D}\phi e^{-S_E(\psi)}
\end{equation}   
with the field measure replaced by a finite product
\begin{equation}
\mathcal{D}\phi = \prod_{n\in\Lambda} d\phi(n).
\end{equation}
The expectation value of an observable is computed as
\begin{equation}
\expval{\mathcal{O}} = \frac{1}{\mathcal{Z}}\int \mathcal{D}\phi e^{-S_E(\phi)}\mathcal{O}(\phi)
\end{equation}
where generally the functional $\mathcal{O}(\phi(\Lambda))$ depends on the whole configuration of fields in the lattice.

%\subsection*{Continuum limit}
%
%A lattice measured observable $m$ has lattice artifacts, namely $a$-dependent corrections
%\begin{equation}
%m(a) = m_\text{phys}(1+\order{a})
%\end{equation}
%depending on the discretization procedure. One is interested in obtaining results for a continuous space-time, eliminating these corrections. Taking this limit also allows for a better comparison with experimentally measured quantities. Hence it is important to know how the observables change with the parameter $a$.
%
%The limit $a\rightarrow 0$ cannot be performed analytical since the functional dependence on both the spacing and volume are not known. Numerically the limit is also not feasible since it is limited by computational power, and the thermodynamic limit ($V\rightarrow \infty, ~N \rightarrow\infty$) which precedes the $a\rightarrow0$ limit is impossible. One is usually left with an extrapolation using fixed volume lattices with decreasing spacing $a$. The reverse can also be done, varying the volume with fixed spacing to study the finite volume dependence. A thorough study of these limits was done in \cite{Oliveira_2012} for the gluon propagator where it is shown that the interplay of both limits is far from trivial.
%
%In section \ref{sec:euclidean formulation} it was pointed that there are certain conditions to allow a contact between the Euclidean and the Minkowski physics. However, we can also worry about the legitimacy of describing continuum physics in a lattice, namely if the non-uniqueness of the action discretization spoils the correct limit. Fortunately the structural correspondence between lattice field theory and statistical mechanics allows to use the concept of \textit{universality} that guarantee the uniqueness limit \cite{kogut}. In fact, the continuum limit of the theory is formally equivalent to the approach to criticality in a general statistical mechanical system \cite{goldenfeldlectures}.
%
%Other than the continuum limit of the action, we could also question if the lattice formulation itself provides a proper description of a general quantum field theory. The Osterwalder-Schrader conditions referred before apply only to the Wick's rotation, thus a proper proof of the positivity condition for the lattice is required. Fortunately, for QCD it was shown in \cite{Luscher_positivity} that transition amplitudes between states are non-negative, and that the associated Hamiltonian has real eigenvalues. These conditions are necessary to construct the Hilbert space with proper physical states. Hence, lattice QCD describes a physical system with the correct continuum limit.


\section{Lattice Chromodynamics}\label{sec:Lattice Chromodynamics}


Having established the basics of the lattice formulation for a generic field theory we may apply it to the theory of strong interactions. We consider only the pure Yang-Mills Lagrangian and so we examine exclusively the discretization of this piece. Although we do not consider matter fields, in the lattice the gluon fields also appear in order to preserve gauge invariance in local gauge transformations, $\psi(n) \rightarrow V(n)\psi(n)$, where $V(n)$ are $SU(3)$ group elements on the lattice sites

In the continuum, we considered the covariant derivative to fix the gauge invariance of the action, this was implemented so as the comparison of fields at different points was to be properly defined. This object was constructed using the concept of a comparator. In the lattice, two neighbouring points have corresponding transformations with $V(n)$ and $V(n+\hat\mu)$, where now $\hat\mu$ is a lattice vector in the direction $\mu$ with length $a$.

In the lattice, we define the group-valued object $U_\mu(n)$ connecting the points $n$ and $n+\hat\mu$. These $SU(3)$ matrices are the fundamental fields in this framework. Since these objects compare fields at neighbouring points, they are oriented and live on the links between lattice sites, therefore are called \textit{link variables}. The inverse direction link variable is given by the adjoint operator $U_\mu^\dagger(n-\hat\mu)$ - the geometrical representation is shown in figure \ref{fig:comparators}. The link variables are defined by their behaviour under a gauge transformation,
\begin{equation}
U_\mu(n) \rightarrow U'_\mu(n) = V(n)U_\mu(n)V^\dagger(n+\hat\mu).
\end{equation}
%
\tikzset{->-/.style={decoration={
			markings,
			mark=at position #1 with {\arrow{>}}},postaction={decorate}}}
%
\begin{figure}[H]
	\begin{center}
		\begin{tikzpicture}
		\draw[->-=.56,line width=1mm] (-1,0) to (-4,0);
		\draw[->-=.56,line width=1mm] (1,0) to (4,0);
		\filldraw [black,very thick] (-1,0) circle (2pt);
		\filldraw [black,very thick] (-4,0) circle (2pt);
		\filldraw [black,very thick] (4,0) circle (2pt);
		\filldraw [black,very thick] (1,0) circle (2pt);
		\draw[-,line width=.4mm] (-1,-0.5) to (-1,0.5);
		\draw[-,line width=.4mm] (-4,-0.5) to (-4,0.5);
		\draw[-,line width=.4mm] (1,-0.5) to (1,0.5);
		\draw[-,line width=.4mm] (4,-0.5) to (4,0.5);
		\draw[-,line width=.4mm] (-4.5,0) to (-4,0);
		\draw[-,line width=.4mm] (4,0) to (4.5,0);
		\draw[-,line width=.4mm] (1,0) to (.5,0);
		\draw[-,line width=.4mm] (-1,0) to (-0.5,0);
		\node[align=center] at (2.5,-1) {$U_\mu(n)$};
		\node[align=center] at (-2.5,-1) {$U_{-\mu} = U_\mu^\dagger(n-\hat\mu)$};
		\node[align=center] at (-4.6,-0.3) {$n-\hat\mu$};
		\node[align=center] at (4.6,-0.3) {$n+\hat\mu$};
		\node[align=center] at (0.7,-0.3) {$n$};
		\node[align=center] at (-0.7,-0.3) {$n$};
		\end{tikzpicture}
	\end{center}
	\caption{Link variable between $n$, $n+\hat\mu$ and $n-\hat\mu$. }
	\label{fig:comparators}
\end{figure}

We want to build the simplest lattice action in a way that the Yang-Mills action is restored when the continuum limit is taken. In the continuum, a gauge invariant object was built through the commutator of covariant derivatives in two directions, which is equivalent to the product of comparators around a square loop. To construct this object we start by defining the product of comparators along a path $\mathcal{P}$ linking $k$ sites between $n_0$ and $n_1$
\begin{equation}
P[U] = U_{\mu_0}(n_0)U_{\mu_1}(n_0+\hat\mu_0)...U_{\mu_{k-1}}(n_1-\hat\mu_{k-1}).
\end{equation}
whose gauge transformation depends only on the endpoints 
\begin{equation}
	P[U] \rightarrow P'[U] = G(n_0)P[U]G^\dagger(n_1).
\end{equation}
If we consider a closed path, i.e. $n_0 = n_i$ and the trace is applied
\begin{equation}
	\Tr P'[U] = \Tr\left(G(n_0)P[U]G^\dagger(n_0)\right) = \Tr P[U],
	\label{eq:gauge invariant trace loop}
\end{equation}
we obtain a gauge invariant object 
Considering the elementary square loop in the plane $\mu - \nu$ -- \textit{plaquette}, see \cref{fig:plaquette} -- the product of group elements around the square reads 
\begin{equation}
U_{\mu\nu}(n) = U_\mu(n)U_\nu(n+\hat\mu)U_\mu^\dagger(n+\hat\nu)U_\nu^\dagger(n).
\label{eq:plaquette}
\end{equation}
%
\begin{figure}[htb!]
	\centering
	\begin{tikzpicture}[scale=0.9, every node/.style={scale=0.9}]
	\draw[->-=.56,line width=.5mm] (-1,1) to (-1,-1);
	\draw[->-=.56,line width=.5mm] (1,1) to (-1,1);
	\draw[->-=.56,line width=.5mm] (1,-1) to (1,1);
	\draw[->-=.56,line width=.5mm] (-1,-1) to (1,-1);
	
	\draw[-=.56,line width=.1mm] (-1,-1.5) to (-1,1.5);
	\draw[-=.56,line width=.1mm] (1,-1.5) to (1,1.5);
	\draw[-=.56,line width=.1mm] (-1.5,-1) to (1.5,-1);
	\draw[-=.56,line width=.1mm] (-1.5,1) to (1.5,1);
	
	\filldraw [black,very thick] (-1,1) circle (2pt);
	\filldraw [black,very thick] (-1,-1) circle (2pt);
	\filldraw [black,very thick] (1,1) circle (2pt);
	\filldraw [black,very thick] (1,-1) circle (2pt);
	
	\node[align=center] at (-1.5,-1.5) {$n$};
	\node[align=center] at (-1.57,1.5) {$n+\hat\nu$};
	\node[align=center] at (2,1.5) {$n+\hat\mu+\hat\nu$};
	\node[align=center] at (2,-1.5) {$n+\hat\mu$};
	
	\node[align=left] at (-2,0) {$U_\nu^\dagger(n)$};
	\node[align=left] at (0,-1.5) {$U_\mu(n)$};
	\node[align=left] at (2.2,0) {$U_\nu(n+\hat\mu)$};
	\node[align=left] at (0,1.5) {$U_\mu^\dagger(n+\hat\nu)$};
	\end{tikzpicture}
	\caption{Schematic representation of the minimal planar lattice loop -  \textit{plaquette} in the plane $\mu - \nu$. }
	\label{fig:plaquette}
\end{figure}%
Due to the form of the continuum action we need a relation between the link variables and the continuum gauge fields $A_\mu(x)$. Hence we require that $U_\mu(n) = U(n,n+\hat\mu) + \order{a}$, establishing a relation between lattice and continuum comparators. For this purpose, we introduce algebra valued lattice gauge fields by
\begin{equation}
U_\mu(n) = e^{iagA_\mu(n+\hat\mu/2)} + \order{a}.
\label{eq:gaugelink_gaugefield}
\end{equation}
We now rewrite \cref{eq:plaquette} using these gauge fields and the Baker-Campbell-Hausdorff formula for the product of exponentials of matrices
\begin{equation*}
e^Ae^B = e^{A+B+\frac{1}{2}[A,B]+ ...}.
\end{equation*}
With this we obtain a relation with the discretized version of the field strength tensor $F_{\mu\nu}(n)$
\begin{align}
U_{\mu\nu} &= e^{ia^2(\partial_\mu A_\nu(n) + \partial_\nu A_\mu(n) + i[A_\mu(n),A_\nu(n)]) + \order{a^3}}  \nonumber \\
&= e^{iga^2F_{\mu\nu}(n) + \order{a^3}}.
\label{eq:lattice_comparator_fieldtensor}
\end{align}
Therefore, to obtain the lattice Wilson action, we consider the sum
\begin{align}
S_\text{G}[U] =& \frac{\beta}{2N}\sum_{n}\sum_{\mu,\nu}\Re\Tr(\mathds{1} - U_{\mu\nu}(n))\\
=&\frac{a^4}{2g^2}\sum_{n}\sum_{\mu,\nu}\Tr(F_{\mu\nu}^2(n))+\order{a^2}.
\label{eq:Wilson action}
\end{align}
which restores the continuum action to order $\order{a^2}$.
It is usual to define the inverse bare lattice couppling $\beta = 2N/g^2$.
%To reach the second line of \eqref{eq:Wilson action} just expand \eqref{eq:lattice_comparator_fieldtensor} in the lattice spacing. The terms of order $\order{a^2}$ vanish when taking the real part - it would vanish with the trace operation regardless, since it involves a single algebra matrix. 
This form of the action considers nearest neighbours interaction. It was formulated firstly by Wilson in 1974 considering also fermions - see \cite{Wilson1974}.

This approximation, disregarding the quarks dynamics is called \textit{quenched approximation}. This scheme has the added benefit of not involving the fermionic discretization which introduces unsolved problems.
Although seemingly drastic, this choice is associated with small errors. The hadronic spectra shows differences around $10$ to $20\%$ relative to the unquenched results \cite{Aoki_2003}. 

\section{Gauge fixing}\label{sec:gauge fixing}


Since no problems arise from an infinite degeneracy of gauge transformations in the lattice, fixing a gauge is not mandatory, however it is beneficial. This is because although physical observables do not depend on the gauge, certain intermediate objects are not gauge invariants. This is the case of the correlation functions, which can be shown to vanish if no gauge is fixed - Elitzur's theorem \cite{Elitzur}.

In this work we consider the Landau gauge. In the continuum this condition is $\partial_\mu A^\mu(x) = 0$, or equivalently $p_\mu A^\mu(p) = 0$ in momentum space. It can be shown that this condition is equivalent to finding the stationary points of the functional\footnote{Changing momentarily to the Minkowski metric with lower and upper indices.},
\begin{equation}
W[A] = \int d^4x\Tr(A_\mu(x)A^\mu(x)).
\end{equation}
This can be seen by considering an infinitesimal gauge transformation $V(x) = \exp(-i\varepsilon H(x))$ applied to the field and using the transformation law \eqref{eq:gaugetransform_infinitesimal}
\begin{equation}
A_\mu(x) \rightarrow A_\mu(x) + \varepsilon(i[H(x),A_\mu(x)] -\partial_\mu H(x)) + \order{\varepsilon^2}. 
\end{equation}
Where $H(x)$ is an hermitian traceless matrix in the Lie algebra of $SU(3)$. If we insert this transformation into the functional, and perform integration by parts, we obtain
\begin{equation}
W[A] \rightarrow W[A] +2\varepsilon\int d^4x\Tr((\partial_\mu A^\mu(x))H(x)) + \order{\varepsilon^2}.
\end{equation}
For $W[A]$ to be a stationary point the $\order{\varepsilon}$ contribution should vanish. Since $H(x)$ is arbitrary, this is equivalent to $\partial_\mu A^\mu(x) = 0$.

This functional can be translated into the lattice formulation, expressing the functional through the gauge group elements instead of the algebra valued fields,
\begin{equation}
W_\text{lat}(x) = -a^2\sum_{n,\nu}\Tr[U_\mu(n) + U_\mu^\dagger(n)].
\end{equation}
We now introduce the gauge transformation $V(n)$ which rotates this functional into the minimum. This can be accomplished by minimizing the functional,
\begin{equation}
F_U[V] = -\frac{1}{VN_dN_c}\sum_{n,\nu}\Tr\left[V(n)U_\mu(n)V^\dagger(n+\hat\mu)\right],
\label{eq:gauge functional lattice}
\end{equation}
where $V$ is the volume of the lattice, $N_d$ and $N_c$ the dimensions and colour number, respectively.

Unfortunately, the situation is not as easy as presented. This is caused by residual ambiguity in the extrema for the functional - this problem arises already in the continuum formulation. Ideally we want the gauge condition to intersect each gauge orbit uniquely. However, Gribov \cite{Gribov_1977} showed that for a non-abelian gauge theory in the Coulomb gauge ($\partial_i A_i(x)=0$) there are equivalent gauge fields in each orbit that also satisfy the condition -- \textit{Gribov copies}. It was later generalized \cite{Killingback_gauge} for an arbitrary $SU(N)$ gauge theory in a 4-dimensional torus\footnote{Corresponding to an hypercubic lattice theory with periodic boundaries.} that no continuous local gauge condition can be found that is free of the Gribov copies.

The presence of the copies implies the existence of various stationary points of the functional \eqref{eq:gauge functional lattice}. Gribov suggested additional constraints to the gauge field configuration space further restricting the integration on the gauge fixing hypersurface. It can be shown that in the lattice these restrictions guarantee the absence of Gribov copies in this region \cite{zwanziger_gribov}. This in turn guarantees the existence of a global minimum of \cref{eq:gauge functional lattice} in the lattice. Numerically, the search is limited to a local minimum -- this was done by the steepest descent method, described in \cite{Fourier_acceleration_method}.

A review of the gauge fixing on the lattice can be found in \cite{GIUSTI_2001}. It is worth referring that the effect of the Gribov copies was studied for the gluon propagator in the lattice \cite{Silva_2004,CUCCHIERI1998841} concluding that its effect are small. In this work we did not consider the effect of the Gribov copies.

\section{Correlation functions from the lattice}

We are interested in computing lattice correlation functions representing the gluon vertices, however the field configurations are generated using the link variables $U_{\mu}(n)$. We need to extract the lattice algebra gluon fields $A_\mu(n)$. To establish this relation, we consider the inverse of \cref{eq:gaugelink_gaugefield}. Expanding the exponential in $a$, the following relation is obtained
\begin{equation}
agA_\mu(x+\hat\mu/2) = \frac{1}{2i}\left[U_\mu(n) - U_\mu^\dagger(n)\right] - \frac{1}{6i}\Tr\left[U_\mu(n) - U_\mu^\dagger(n)\right]
\label{eq:gaugefield_lattice}
\end{equation}
where trace term in \eqref{eq:gaugefield_lattice} guarantees that the gauge field $A_\mu$ is traceless.
We work with momentum correlation functions. For this end we consider the discrete Fourier transform defined before,
\begin{equation}
A_\mu(p) = \sum_{x}e^{-ip\cdot(x+\hat\mu/2)}A_\mu(x+\hat\mu/2)
\label{eq:gauge transform lattice}
\end{equation}
with $p=2\pi n/aL,~n\in[-L/2+1,L/2]$. 
%\footnote{The Landau condition in the lattice is $\sum_{\mu}(A_\mu(x+\hat\mu) - A_\mu(x)) = 0$. I one were to use a usual Fourier transform, the condition in momentum space would read 
%$$ \sum_{\mu}[\cos p_\mu - 1 - i\sin p_\mu]A_\mu(p) = 0 $$
%while if one were to use the improved 
%$$ \sum_{\mu}2\sin(p_\mu/2) A_\mu(p) = 0$$
%which in the continuum limit recovers the condition to $\order{a^2}$, while the first to $\order{a}$} 

The gluon two point function is extracted from the average over the gauge field configurations by
\begin{equation}
\expval{A_{\mu_1}^{a_1}(p_1)A_{\mu_2}^{a_2}(p_2)} = D_{\mu_1\mu_2}^{a_1a_2}(p_1)V\delta(p_1+p_2).
\end{equation}
with the volume of the lattice $V$.
In \cref{subsec:expectation values in the lattice} we will see how these averages are performed in the lattice in order to extract the Green's functions.

In the framework we perform simulations we have access to algebra valued gauge fields $A_\mu(p)$ from \cref{eq:gaugefield_lattice,eq:gauge transform lattice}, and not to each colour element $A_\mu^a(p)$. In order to extract form factors, we need to form a scalar from these quantities. For this a colour trace is considered. Considering the usual continuum tensor description for the gluon propagator \cref{eq:full_continuum_propagator}, the form factor $D(p^2)$ is obtained by the following operation
\begin{equation}
D(p^2) = \frac{2}{(N_c^2-1)(N_d-n)}\sum_{\mu}\expval{\Tr\left[A_{\mu_1}(p)A_{\mu_2}(-p) \right]}
\label{eq:continuumtensor_extraction}
\end{equation}
where $n=0$ if $p=0$ or $1$ otherwise.
 
For the gluon propagator, the analysis of the colour indices is rather simple since only $\delta^{a_1a_2}$ can be used, independently of the Lorentz tensor structure.
For the three and four gluon vertices we again have access to the product of algebra valued gauge fields to which we apply the trace in the group space to obtain a scalar in this space,
\begin{align}
&\expval{\Tr\left[A_{\mu_1}(p_1)A_{\mu_2}(p_2)A_{\mu_3}(p_3)\right]} = V\delta(\sum_{i}p_i)G_{\mu_1\mu_2\mu_3}(p_1,p_2,p_3) 
\label{eq:3gluon_correlation_trace}\\
&\expval{\Tr\left[A_{\mu_1}(p_1)A_{\mu_2}(p_2)A_{\mu_3}(p_4)A_{\mu_4}(p_4)\right]} = V\delta(\sum_{i}p_i)G_{\mu_1\mu_2\mu_3\mu_4}(p_1,p_2,p_3,p_4)
\label{eq:4gluon_correlation_trace}
\end{align}
where the $G$'s represent the Green's functions with colour indices absorbed by the trace operation and whose form depends on the tensor basis considered. These tensor bases will be the subject of discussion in \cref{chap:tensorbases}. 

\section{Computational aspects}

\subsection{Expectation values in the lattice}\label{subsec:expectation values in the lattice}

In the Euclidean formulation of the theory, the expectation value of some field dependent operator is obtained as
\begin{equation}
\expval{\mathcal{O}} = \frac{1}{\mathcal{Z}}\int\mathcal{D}U \mathcal{O}(U)e^{-S_E[U]}
\label{eq:euclidean_expect_value}
\end{equation}
which even if we consider a finite lattice, it is still an integral over infinite configurations. To obtain numerical results we must consider only a finite number of field configurations. The way to do this is by importance sampling considering the weight of the Boltzmann factor in the Euclidean action.

One resorts to Monte Carlo methods \cite{morningstar2007monte}. A set of gauge field configurations\footnote{ By a gauge field configuration we mean that each site of the lattice is attributed a value of the field $U$, i.e. a Lorentz vector of $SU(3)$ matrices.} $\{U_i\},~i=1,...,n$ is generated according to the probability distribution 
\begin{equation}
	 P(U) = e^{-S_E(U)}/\mathcal{Z}.
\end{equation}
The sequence of is obtained by a Markov process which generates the configurations, one after another according to a transition amplitude $P(U_i\rightarrow U_j)$ depending solely on the predecessor configuration. This transition amplitude should create a set distributed according to $P(U)$ in the large $n$ limit. The precise form of the amplitudes depends on the chosen method \cite{Rothe}. When the set $\{U_i\},~i=m,...,n$ is properly distributed by $P(U)$, it is said to be \textit{thermalized}. The set $\{U_i\},~i=1,...,N$ used for the averaging is chosen from the thermalized set.
The configurations considered in this thesis were obtained using a combination of the over-relaxation and the heat bath methods according to \cite{anthony_2016}.

With a finite number of configurations following the $\exp(-S_E(U))/\mathcal{Z}$ probability distribution, the expectation value \eqref{eq:euclidean_expect_value} is estimated by the sample mean
\begin{equation}
\bar{\mathcal{O}} = \frac{1}{N}\sum_{i=1}^{N}\mathcal{O}(U_i)
\end{equation} 
which corresponds to the complete ensemble average $\expval{\mathcal{O}}$ in the large $N$ limit.

If we admit that all configurations in the sample are statistically independent, having no correlations, then the sample average is normally distributed around the true expectation value, and the error estimate would be $\expval{\mathcal{O}} = \bar{\mathcal{O}}+1/\sqrt{N}$. This estimate is too optimistic since the process of generating the configurations introduces correlations among them \cite{montvay_1994}. To estimate the uncertainty of an average over the configurations without assuming a statistical distribution inherent to the variables, we use the \textit{Bootstrap method}, delineated below.

\subsection{Bootstrap method}\label{sec:bootstrap}

In this thesis, all statistical errors are obtained through the bootstrap method. The bootstrap is a distribution independent method that can be applied to estimate the statistical error of any quantity $\mathcal{S}$, disregarding its functional form -- for a complete review of the method, see \cite{bootstrap_Efron}. 

To start, consider a given initial sample of $N$ elements $\{U_i\},~i=1,...,N$ obtained from an unknown distribution, which in our case corresponds to the gauge field configurations. We are interested in obtaining the statistical error associated to a quantity $\mathcal{S}(U)$. In this work this quantity corresponds to a mean value of some quantity over the configurations.

The method consists in considering the \textit{empirical distribution} for the original sample, assigning the probability $1/N$ to each of the observed elements. A bootstrap sample is constructed by random sampling with replacement from this probability distribution. We obtain $N_b$ random samples $U_b^j=(U^j_1,...,U^j_N)$ from the original, of the same size $N$. For each sample $i$, the quantity is computed to be $\mathcal{S}^j \equiv \mathcal{S}(U^j)$. The idea of the method is that now, we have a proper random variable $\mathcal{S}^j$ with a known distribution -- the empirical. 

We want to obtain confidence intervals without assuming the underlying distribution. 
%The bootstrap method to build the confidence region does not require consulting a model dependent table for the intervals, for it builds the appropriate intervals for the data at hand. 
The bootstrap method provides asymmetric boundaries around the expectation value.
Having $N_b$ values $\mathcal{S}^j$, from which we obtain $\bar{\mathcal{S}}$, the upper and lower errors are estimated using confidence intervals,
\begin{align}
\sigma_\text{up} = \mathcal{S}_\text{up}-\bar{\mathcal{S}}, && \sigma_\text{down} = \bar{\mathcal{S}} - \mathcal{S}_\text{down}
\end{align}
where $\mathcal{S}_\text{up}$ and $\mathcal{S}_\text{down}$ are found in a way that they satisfy
\begin{align}
\frac{\#\{\mathcal{S}^j < \mathcal{S}_\text{up} \}}{N_b} = \frac{1+C}{2}, &&
\frac{\#\{\mathcal{S}^ j < \mathcal{S}_\text{down} \}}{N_b} = \frac{1-C}{2}
\end{align}
where $C$ is the coefficient chosen for the confidence interval, $C\in[0,1]$ and $\#\{\}$ represents the cardinality of a given set. 

%To better understand these relations, look at the one for $\mathcal{S}_\text{down}$, and consider a situation with 1000 bootstrap samples and $C = 0.6$. Firstly, $C$ represents the probability of the interval around the estimator $\bar{\mathcal{S}}$ we compute - in this case $60\%$. The ratio $(1-C)/2 = 0.2\%$ gives the probability below the lowest limit. To find this limit, we find the $1000\times(1-C)/2 = 200$th highest value of the ordered $\mathcal{S}^j$, which corresponds to $\mathcal{S}_\text{down}$. The procedure is similar for the upper limit, considering the $1000\times(1+C)/2 = 800$th highest sample.

In this thesis, $C$ was chosen to be $C = 0.675$ representing a $67.5\%$ probability of the true estimator falling in the interval. The uncertainty was taken to be the largest of the two errors. For all results obtained, a factor of 10 is considered to generate the random samples from the original.


\subsection{Setting the scale}\label{sec:settingthescale}

When a set of lattice configurations are generated, every quantity obtained by averaging over the set is dimensionless. The values are given in terms of the lattice spacing $a$. To obtain real physical values we need to set this scale by choosing a correct value for $a$ which is not an input parameter of the theory. 

To do this we match a given dimensionless lattice computed object (say, $am_g$) with an experimental value ($m_{g,\text{phys}}$) at a given energy scale. The lattice spacing is then obtained by
\begin{equation}
a = \frac{am_g}{m_{g,\text{phys}}}.
\end{equation} 

In our case, this procedure was done using the static potential between two colour charges, which can be computed in the pure Yang-Mills formulation (see \cite{Gattringer2010} for a complete analysis). The trace of comparators around a closed loop $\mathcal{L}$ 
\begin{equation}
	W_\text{L} = \Tr\left(\prod_{(n,\mu)\in\mathcal{L}}U_\mu(n)\right)
\end{equation}
is a gauge invariant object - see \cref{eq:gauge invariant trace loop}. Its expectation value can be related to the interaction between two colour charges in the static limit where their masses become infinite,
\begin{equation}
\expval{W_\text{L}} = \sum_{n}\left|\psi_k(\mathbf{m})\bar\psi_k(\mathbf{n})\right|^2 e^{-an_4E_k}
\end{equation}
where $n_4$ represents the time direction in the lattice, $k$ labels the energy eigenstates and $\mathbf{m}$, $\mathbf{n}$ two spatial points of the lattice with the same time coordinate $n_4$.
The first term of this sum, corresponding to the lowest energy is shown \cite{Gattringer2010} to be associated with the static quark-antiquark pair, therefore $E_0$ will correspond to the inter quark potential,
\begin{equation}
E_0 = V(r),~r=a|\mathbf{m}-\mathbf{n}|.
\end{equation}
With this, we can obtain the potential through the large $n_4$ behaviour of the loop expectation value, which suppresses the remaining higher energy contributions,

\begin{equation}
\expval{W_\text{L}} \propto e^{-an_4V(r)}\left(1+\order{e^{-an_4\Delta E}}\right)
\end{equation}
where $\Delta E$ corresponds to the energy gap between $V(r)$ and the first excited energy level of the pair.


The quark potential is generally modelled by $V(r) = A/r + \sigma r$, where the first term corresponds to a Couloumb term, while the second is a pure QCD contribution. $\sigma$ is called the \textit{string tension}, and by fixing its value with an experimental result, the scale $a$ is set. The lattice spacing of the configuration ensembles used in this work was computed from the string tension data in  \cite{Bali_coulingconstant}.

